Robustness from Simple Classifiers

Despite the vast success of Deep Neural Networks in numerous application domains, it has been shown that such models are not robust i.e., they are vulnerable to small adversarial perturbations of the input. While extensive work has been done on why such perturbations occur or how to successfully defend against them, we still do not have a complete understanding of robustness. In this work, we investigate the connection between robustness and simplicity. We find that simpler classifiers, formed by reducing the number of output classes, are less susceptible to adversarial perturbations. Consequently, we demonstrate that decomposing a complex multiclass model into an aggregation of binary models enhances robustness. This behavior is consistent across different datasets and model architectures and can be combined with known defense techniques such as adversarial training. Moreover, we provide further evidence of a disconnect between standard and robust learning regimes. In particular, we show that elaborate label information can help standard accuracy but harm robustness.

==> attacks.tex <==
\section{Attacks}

While there exist well-known techniques, such as PGD for attacking a multiclass neural network, it is not immediately obvious what is the best way to attack the aggregation of binary classifiers that we propose in this paper. We tried the following methods:

\textbf{Attack all arms independently and select the best attack.} Since the proposed architecture consists of several simpler classifiers/arms, a natural attack is to construct individual adversarial examples for each arm of the aggregation. Subsequently, we select one of the examples that is misclassified arbitrarily, assuming that such an example exists.

\textbf{Attacking a combination of arms.} Another promising attack would be to try to attack the arm with the highest and the second highest scores simultaneously, aiming to decrease the score of the highest arm and increase the score of the second highest, hence inducing misclassification. In order to do that, we average the gradients of these two arms and use this gradient in our PGD procedure. The PGD update is the following where $L_1$ and $L_2$ correspond to the loss of the best and the second best arms respectively: $x^{k+1} = \Pi_{\mathcal{B}}\left(x^{k} + \frac{\eta}{2}\nabla_xL_1(x^k, y) + \frac{\eta}{2}\nabla_xL_2(x^k, y) \right)$

\textbf{Attacking the binary aggregation in a continuous way.} For this attack we connect the outputs of all the arms with a softmax layer as shown in Figure~\ref{fig:softmax}. Subsequently, we apply PGD on this new network. The intuition behind this attack is that, Since $\texttt{softmax}$ is a continuous and differentiable relaxation of the $\texttt{max}$ function---our prediction function---this attack essentially serves as a tractable way to attack a differentiable version of the aggregation using gradient-based methods.

\textbf{Attacking the top two arms of binary aggregation in a continuous way.} This approach is a combination of the methods described before. We connect only the arms with the best and the second best scores for each image with a softmax layer in order to find a smooth way to decrease the score of the best arm and increase the score of the second best using gradient-based methods.




% We report on the accuracy of the attack methods we described in Table~\ref{table:attacks}. A sample of these runs can be found in Figure~\ref{fig:attacks}.

% \begin{figure}[t]
% \begin{center}
%   \includegraphics[width=.45\textwidth]{tmp_figures/attacks.pdf}
% \end{center}
% \label{fig:attacks}
% \caption{Attacks on the aggregated classifiers and the multi-class model.}
% \end{figure}

% \begin{figure}[t]
% \begin{center}
%   \includegraphics[width=.45\textwidth]{tmp_figures/transfer.pdf}
% \end{center}
% \label{fig:transfer}
% \caption{Transferability of adversarial examples from the multi-class to the binary aggregation model. In the targeted case, each image is transformed towards the second most likely class predicted by the aggregation model.}
% \end{figure}
